Top quark physics in the Large Hadron Collider era

We explore various aspects of top quark phenomenology at the Large Hadron Collider and proposed future machines. After summarising the role of the top quark in the Standard Model (and some of its well-known extensions), we discuss the formulation of the Standard Model as a low energy effective theory. We isolate the sector of this effective theory that pertains to the top quark and that can be probed with top observables at hadron colliders, and present a global fit of this sector to currently available data from the LHC and Tevatron. Various directions for future improvement are sketched, including analysing the potential of boosted observables and future colliders, and we highlight the importance of using complementary information from different colliders. Interpretational issues related to the validity of the effective field theory formulation are elucidated throughout. Finally, we present an application of artificial neural network algorithms to identifying highly-boosted top quark events at the LHC, and comment on further refinements of our analysis that can be made.

==> professor-content.tex <==

\newpage
\appendix
\section{The {\sc{Professor}} fitting method}
Throughout this thesis we have made extensive use of the {\sc{Professor}} Monte Carlo tuning/validation software to tackle the problem of parameter fitting in multidimensional parameter spaces of Wilson coefficients. We discussed the method briefly in chapters 3 and 4, but to keep the focus of the main text on physics, we have postponed an extended discussion of our fit methodology to this appendix\footnote{A full discussion can of course be found in the original paper, but since we utilise an adapted version of the tool in this thesis, we reproduce the relevant parts of that discussion here.}.

\section*{Interpolation based tuning}
When sampling the parameter space of a theory, unless the region of interest occupies a very small volume of the total theory `hypercube' or the parameter space has a very small number of dimensions, approximations must be made to keep the computational complexity of the sampling under control. For instance, the na\"ive \emph{brute force} approach would be to sample on a grid, i.e. to generate the theory predictions at parameter space points on a grid. This approach will not scale well in the number of parameters, however. Requiring an accuracy of $N$ sample points per dimension $d$ leads to a total running time \ord{\mathnormal{N^d}}, i.e. this approach has exponential complexity.  


